A Tighter Bound for the Determinization of Visibly Pushdown Automata

Visibly pushdown automata (VPA), introduced by Alur and Madhusuan in 2004, is a subclass of pushdown automata whose stack behavior is completely determined by the input symbol according to a fixed partition of the input alphabet. Since its introduce, VPAs have been shown to be useful in various context, e.g., as specification formalism for verification and as automaton model for processing XML streams. Due to high complexity, however, implementation of formal verification based on VPA framework is a challenge. In this paper we consider the problem of implementing VPA-based model checking algorithms. For doing so, we first present an improvement on upper bound for determinization of VPA. Next, we propose simple on-the-fly algorithms to check universality and inclusion problems of this automata class. Then, we implement the proposed algorithms in a prototype tool. Finally, we conduct experiments on randomly generated VPAs. The experimental results show that the proposed algorithms are considerably faster than the standard ones.

==> eptcsdata.tex <==
\providecommand{\event}{Axel Legay and Azadeh Farzan (Eds.): International Workshop on Verification of Infinite-State Systems (INFINITY 2009)}
\providecommand{\volume}{10}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{62}
\providecommand{\eid}{5}
\pdfoutput=1

